NAAS: Neural Accelerator Architecture Search

Data-driven, automatic design space exploration of neural accelerator architecture is desirable for specialization and productivity. Previous frameworks focus on sizing the numerical architectural hyper-parameters while neglect searching the PE connectivities and compiler mappings. To tackle this challenge, we propose Neural Accelerator Architecture Search (NAAS) which holistically searches the neural network architecture, accelerator architecture, and compiler mapping in one optimization loop. NAAS composes highly matched architectures together with efficient mapping. As a data-driven approach, NAAS rivals the human design Eyeriss by 4.4x EDP reduction with 2.7% accuracy improvement on ImageNet under the same computation resource, and offers 1.4x to 3.5x EDP reduction than only sizing the architectural hyper-parameters.

==> text/float/figures/eval/has/onenet.tex <==
\begin{figure*}[t]
\centering
    \includegraphics[width=0.9\linewidth]{figures/results/has/has-onenet.pdf}
    \caption{Speed up and energy savings when \naas searches hardware and mapping for each network independently with baseline hardware resources. For instance, using same \#PEs and SRAM size as Shidiannao, \naas is able to offer an specialized hardware for VGG-16 with 2.1$\times$ speedup than Shidiannao itself.}
    \label{fig:has-onenet}
\end{figure*}

==> text/float/figures/nhs/enhas.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/nhs/enhas.pdf}
    \caption{Integrating \naas with neural architecture search.}
    \label{fig:enhas}
\end{figure}

==> text/float/figures/nhs/has/ehas.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/nhs/ehas.pdf}
    \caption{\NAAS.}
    \label{fig:ehas}
\end{figure}

==> text/float/tables/eval/has-compare.tex <==
% Table generated by Excel2LaTeX from sheet 'HAS.B1.d256'
\begin{table}[t]
  \centering
  \caption{Machine learning based hardware architecture search (\has) achieves human performance optimizing the energy-delay product (EDP) with good sample efficiency (batch=16).}
  \scalebox{0.8}{
    \begin{tabular}{c|cccc}
    \toprule
    \multirow{2}[2]{*}{} & Grid  & Random & Bayesian & \multirow{2}[2]{*}{HAS} \\
          & Search & Search & Optimization &  \\
    \midrule
    \# Samples & 250   & 2048 & 2048  & 240 \\
    EDP Reduction & 1.00\X     & 1.05\X  & 0.90\X   & 1.16\X \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:has}%
\end{table}%


==> text/float/tables/eval/platform.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
  \renewcommand*{\arraystretch}{1.15}
  \caption{Hardware resources and design space for \ehas.}
  \scalebox{0.68}{
\begin{tabular}{cc|ccccc}
    \toprule
    % \textbf{Chip} & \textbf{Eyeriss~\cite{chen2016eyeriss}} & \textbf{BitFusion~\cite{sharma2018bitfusion}} & \textbf{SpArch~\cite{zhang2020sparch}}  \\
    \multicolumn{2}{c}{\textbf{Source}} & \textbf{Eyeriss} & \textbf{Shidiannao} & \textbf{NVDLA256} & \textbf{NVDLA1024} & \textbf{EdgeTPU}
    \midrule
    \multirow{3}[1]{*}{\textbf{Baseline Resources}}
    \textbf{\# PEs} & 168 & 64 & 256 & 256 & 4096 \\
    \textbf{SRAM (KB)} & 194 & 288 & 256 & 256 & 8192 \\
    \textbf{Bandwidth (GB/s)} & 12 & 12 & 5 & 15 & 12 \\
    \midrule
    \multicolumn{4}{1}{*}{\textbf{Search Space}}
    
    
    \textbf{Chip} & \textbf{Eyeriss} & \textbf{BitFusion} & \textbf{SpArch}  \\
    \midrule
    \multirow{3}[1]{*}{\textbf{Characteristics}} & DL Arch & DL Arch & SpMM Arch \\
     & Row Stationary  & Systolic Array & Streaming Merger\\
     & 16-b MAC  & 2/4/8/16-bit MAC & Floating-Point MAC\\
    \midrule
    \textbf{\# PEs} & 12$\times$14~=~168 & 16$\times$32~=~512 & 16 \\
    \textbf{SRAM (KB)} & 194 & 164 & 975 \\
    \midrule
    \textbf{Chip Area (mm$^2$)} & 3.60 & 2.69 & 28.49 \\
    % \midrule
    % \textbf{Design Area} & \multirow{2}[1]{*}{-} & Eyeriss Chip Area & \multirow{2}[1]{*}{-} \\
    % \textbf{Constraints (mm$^2$)} & & 4 mm$^2$ &  \\
    \bottomrule
    \multicolumn{4}{l}{* Eyeriss is projected from 65nm to 45nm. Each Eyeriss PE contains a 16b multiplier} \\
    \multicolumn{4}{l}{* Each BitFusion PE equals a 8b multiplier} \\
    \end{tabular}%
    }
  \label{tab:platform}%
\end{table}%

